Universally Composable Simultaneous Broadcast against a Dishonest Majority and Applications

Simultaneous broadcast (SBC) protocols [Chor et al., FOCS 1985] constitute a special class of broadcast channels which have proved extremely useful in the design of various distributed computing constructions (e.g., multiparty computation, coin flipping, e-voting, fair bidding). As with any communication channel, it is crucial that SBC security is composable, i.e., it is preserved under concurrent protocol executions. The work of [Hevia, SCN 2006] proposes a formal treatment of SBC in the Universal Composability (UC) framework [Canetti, FOCS 2001] and a construction secure assuming an honest majority. In this work, we provide a comprehensive revision of SBC in the UC setting and improve the results of [Hevia, SCN 2006]. In particular, we present a new SBC functionality that captures both simultaneity and liveness by considering a broadcast period such that (i) within this period all messages are broadcast independently and (ii) after the period ends, the session is terminated without requiring participation of all parties. Next, we employ time-lock encryption (TLE) over a standard broadcast channel to devise an SBC protocol that realizes our functionality against any adaptive adversary corrupting up to all-but-one parties. In our study, we capture synchronicity via a global clock [Katz et al., TCC 2013], thus lifting the restrictions of the original synchronous communication setting used in [Hevia, SCN 2006]. As a building block of independent interest, we prove the first TLE protocol that is adaptively secure in the UC setting, strengthening the main result of [Arapinis et al., ASIACRYPT 2021]. Finally, we formally exhibit the power of our SBC construction in the design of UC-secure applications by presenting two interesting use cases: (i) distributed generation of uniform random strings, and (ii) decentralized electronic voting systems, without the presence of a special trusted party.

==> related.tex <==
\section{Related Work}\label{sec:related}

\subsection{Broadcast channels}\label{subsec:related_BC}
\begin{itemize}
    \item In~\cite{HirtZ10}, it is shown that 
    \begin{enumerate}
        \item The (strong) \emph{broadcast functionality} $\mc{F}_\msf{BC}$ can be realized without setup iff $t<\frac{n}{3}$ parties are corrupted (cf. \cite[Corollaries 1 and 3]{HirtZ10}).
       \item $\mc{F}_\msf{BC}$ can be realized using a signature setup iff $t\leq\frac{n}{2}$ are corrupted (cf.~\cite[Corollaries 4 and Lemma 8]{HirtZ10}).
       \item The \emph{unfair broadcast functionality} $\mc{F}_\msf{UBC}$ can be realized by using a signature setup for $t<n$ corrupted parties (cf.~\cite[Lemma 4]{HirtZ10}).
    \end{enumerate}
    As observed in~\cite{GarayKKZ11}, the Hirt-Zikas result relies on a very strong assumption regarding the adversary; namely, that the adversary has the ability to corrupt parties \emph{in the middle of a round}, in between sending messages to two other parties in the network.
    \item In~\cite{GarayKKZ11}, it is shown that
    \begin{enumerate}
        \item The Hirt-Zikas impossibility result does not apply in the synchronous model with \emph{atomic message delivery}, i.e.,  messages sent by honest parties within any given round are delivered atomically to all other parties. Still they consider \emph{rushing} corrupted parties, i.e., the adversary may receive its messages in some round before having to send any of its own.
        \item In the atomic model, $\mc{F}_\msf{BC}$ can be realized in the $\mc{F}_\msf{UBC}$-hybrid model for $t<n$. Given~\cite[Lemma 4]{HirtZ10}, we get that $\mc{F}_\msf{BC}$ can be realized by using a signature setup for $t<n$ corrupted parties.
    \end{enumerate}
    The functionality $\mc{F}_\msf{UBC}$ is called relaxed broadcast in~\cite{GarayKKZ11}.
    \item In~\cite{CGZ21}, it is shown that in the non-atomic model (like in~\cite{HirtZ10})
    \begin{enumerate}
        \item For $t>\frac{n}{2}$, $\mc{F}_\msf{BC}$ cannot be realized by solely utilizing TLPs or solely utilizing programmable ROs (cf.~\cite[Theorem 4 and Corollary 15]{CGZ21}).
        \item By utilizing TLPs and programmable ROs, $\mc{F}_\msf{BC}$ can be realized in the $\mc{F}_\msf{UBC}$-hybrid model for $t<n$ (cf.~\cite[Theorem 5]{CGZ21}). Given~\cite[Lemma 4]{HirtZ10}, we get that $\mc{F}_\msf{BC}$ can be realized for $t<n$ corrupted parties by using a signature setup, a TLP, and a programmable RO.
    \end{enumerate}
    \item In SBC, the goal is that no sender can decide its broadcast message based on the values broadcast by the other parties. In~\cite{Hevia06}, a UC definition of SBC is provided. The construction in~\cite{Hevia06} utilizes Verifiable Secret Sharing and is proven UC secure against computationally-unbounded adaptive adversaries assuming an honest majority ($t<\frac{n}{2}$) and private channels. Realization is in the $(\mc{F}_\msf{SMT},\mc{F}_\msf{SYN},\mc{F}_\msf{UBC})$
-hybrid model, where $\mc{F}_\msf{SMT}$ and $\mc{F}_\msf{SYN}$ denote the \emph{secure message transmission} and \emph{synchronous communication} functionalities introduced in~\cite{UC}. As shown in~\cite{KatzMTZ13}, $\mc{F}_\msf{SYN}$ has limitations as it does not provide the guarantees expected of a synchronous network (specifically, termination). These limitations are lifted when relying on a (global) clock functionality~\cite{KatzMTZ13}, as we do in our setting. Besides, $\mc{F}_\msf{SMT}$ can be realized assuming a PKI (e.g., via the certification functionality in~\cite{Canetti04}).

\end{itemize}
\TZ{So, it appears that~\cite{CGZ21} also assumes PKI to realise $\mc{F}_\msf{UBC}$. It seems that in order to transfer the result of~\cite{CGZ21} in our UC setting, we have to adopt the non-atomic model. If we stick to static, then we get no interesting results, as the atomic model (which is stronger model than the static one) considered in~\cite{GarayKKZ11}, already gives a realization assuming only PKI (signatures).}
\MA{What about the relation of simultaneous broadcast with BC. Claim: BC is not enough for CRS, while simultaneous is.}

\subsection{Resource-restricted cryptography (RRC)}\label{subsec:related_RRC}

RRC was introduced in~\cite{GarayKOPZ20}. The authors show that
\begin{enumerate}
    \item The impossibility result of~\cite{Borderding96}   can be circumvented in the RRC setting. According to~\cite{Borderding96}, no Broadcast protocol exists for $t\geq\frac{n}{3}$ even when using local authentication (i.e., signing but no PKI, so that impersonation is not possible but the adversary can send different public keys to parties), CRS and/or a RO. However, in~\cite[Lemma 2 and Corollary 4]{GarayKOPZ20}, via the use of the wrapper $\mc{W}^q(\mc{F}_\msf{RO})$ (that is applied to implement a communication-restricted network) and CRS, $\mc{F}_\msf{auth}$, $\mc{F}_\msf{sig}$ \TZ{What is the difference between the two functionalities? It seems that $\mc{F}_\msf{auth}$ refers to PKI while $\mc{F}_\msf{sig}$ to local authentication}, we get a protocol that invalidates the proof of~\cite{Borderding96}.
    \item They show that MPC for $t<\frac{n}{2}$ is feasible assuming a communication-restricted network (by $\mc{W}^q(\mc{F}_\msf{RO})$), $\mc{F}_\msf{SC}$ (the secure functionality that can be realised by $\mc{F}_\msf{auth}$) and $\mc{F}_\msf{sig}$ (cf.~\cite[Theorem 8]{GarayKOPZ20}.
    
\end{enumerate}

\subsection{Modelling time in UC}
In this work we build fair broadcast from time-lock encryption and unfair broadcast. Here we briefly explain why we do not use the TARDIS model of \cite{BaumDDNO21}.

In \cite{BaumDDNO21}, a framework for modelling time within UC without a global clock is proposed, providing a UC-abstraction of the time-lock assumption, which is used to build UC-secure time-lock puzzles.
%relies on the generic-group model rather than the global clock assumption.
%This is in contrast to \cite{ALZ21}, which builds a time-lock encryption scheme using the global clock assumption instead.

One of our contributions is to provide a UC adaptation of the stand-alone unfair broadcast functionality provided by Cohen et al. in \cite{CGZ21}.
In \cite{CGZ21}, the  authors use a synchronous communication model, and hence it is natural for us to utilise the global clock functionality in our TLE scheme when building fair broadcast. 
%By using used in \cite{ALZ21}.

Furthermore, using the TLE scheme of  \cite{ALZ21} (described in Section \ref{subsec:background_TLE}) allows us to avoid the generic-group assumption, keeping the assumptions used at a minimum.
